A High-Frequency Load-Store Queue with Speculative Allocations for High-Level Synthesis

Dynamically scheduled high-level synthesis (HLS) enables the use of load-store queues (LSQs) which can disambiguate data hazards at circuit runtime, increasing throughput in codes with unpredictable memory accesses. However, the increased throughput comes at the price of lower clock frequency and higher resource usage compared to statically scheduled circuits without LSQs. The lower frequency often nullifies any throughput improvements over static scheduling, while the resource usage becomes prohibitively expensive with large queue sizes. This paper presents a method for achieving dynamically scheduled memory operations in HLS without significant clock period and resource usage increase. We present a novel LSQ based on shift-registers enabled by the opportunity to specialize queue sizes to a target code in HLS. We show a method to speculatively allocate addresses to our LSQ, significantly increasing pipeline parallelism in codes that could not benefit from an LSQ before. In stark contrast to traditional load value speculation, we do not require pipeline replays and have no overhead on misspeculation. On a set of benchmarks with data hazards, our approach achieves an average speedup of 11$\times$ against static HLS and 5$\times$ against dynamic HLS that uses a state of the art LSQ from previous work. Our LSQ also uses several times fewer resources, scaling to queues with hundreds of entries, and supports both on-chip and off-chip memory.

==> Figures/LSQQueues.tex <==


\begin{figure}[t!]
\centering
\subfloat[Store Allocation]{\includegraphics[width=0.24\textwidth]{Figures/st_alloc.pdf}%
\label{fig:StoreAlloc}}%
\hfill%
\subfloat[Store Commit]{\includegraphics[width=0.24\textwidth]{Figures/st_commit.pdf}%
\label{fig:StoreCommit}}%
\vfill%
\subfloat[Load Allocation]{\includegraphics[width=0.39\textwidth]{Figures/ld_alloc.pdf}%
\label{fig:LoadAlloc}}%
\vfill%

\caption{The entries held by the shift-registers in our load-store queue.}

\label{fig:LSQQueues}
\end{figure}



==> Figures/TableDetailsBenchmark.tex <==
\begin{table}[!t]

% increase table row spacing, adjust to taste
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{1.8pt}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
\caption{}
\label{table:codeDescription}
\centering
% Some packages, such as MDW tools, offer better commands for making tables
% than the plain LaTeX2e tabular which is used here.
\begin{tabular}{l | ccccc  }
\hline
\thead{Code} & \thead{Loads} & \thead{Stores} & \thead{Loop IIs} & \thead{Dynamatic store\\ queue size} & \thead{Our allocation\\queue size} \\
% \multirow{2}{*}{\textbf{Code}} & \multirow{2}{*}{\textbf{Loads}} & \multirow{2}{*}{\textbf{Stores}} & \multirow{2}{*}{\textbf{Loop IIs}} & \multicolumn{2}{c}{\textbf{Store queue size}} \\
% & &  & & Dyn & Ours \\
\hline
histogram & 1 & 1 & 2 & 16 & 4 \\
getTanh & 1 & 1 & 56, 1, 1 & 32 & 58 \\
getTanhDouble & 1 & 1 & 13 & 32 & 15 \\
vecTrans & 1 & 1 & 30 & 32 & 32 \\
spmv & 2 & 2 & 1, 9 & 16 & 11 \\
chaosNCG & 2 & 2 & 74 & 8 & 78 \\
BNN & 2 & 2 & 1, 2, 2 & 4 & 4 \\
matching & 2 & 2 & 7 & 16 & 9 \\
floydWarshall & 3 & 1 & 6 & 8 & 8 \\



\end{tabular}

\end{table}

==> rebuttal_old.tex <==
R1:
1a: Our LSQ and compiler passes can be used in any static HLS compiler. In the evaluation, “Intel HLS” is the baseline without our compiler passes and LSQ; “Our work” is with both.
1b: Our LSQ design scales to DRAM because the memory it protects can reside in DRAM, and the only parameter that needs changing is the commit queue size. The actual LSQ logic is still on-chip. We will clarify this.
2a: The size of the allocation shift-register only affects throughout, sec Vc shows how to optimize it. Table II shows the relationship between queue size, frequency, and area. 
2bcd: Sec IVa describes the sizing of the commit shift-register (equal to store latency), and the LSQ load/store execution model. We will highlight this more, together with how the compiler generates the LSQ.
3: We first introduce dynamic scheduling because it enables the use of LSQs. LSQ background is discussed in sec IIc, but we agree that it should be moved forward to highlight it as the focus of the paper.

R2:
1: The address-generating loop is fully decoupled and contains only instructions that generate addresses. We will make this clearer in the paper.
2: The compiler never sequentializes LSQ accesses. Program order is recovered inside the LSQ using tags. The interleaving of misspeculated and actual accesses can be arbitrary, the compiler ensures the right order (alg1 and the proof in sec Vb). Roll-ups are not needed, because only address allocations are speculated – on misspeculation they are discarded. We will clarify this.
3: We do have results for sorting algorithms – their speculation intensity is similar to the maximalMatching benchmark. We will include them. 

R3:
1: The difference between existing CAM-based schemes and our LSQ are discussed in sec IIc. Compared to the single-cycle CAM check in Dynamatic, our logic is spread across cycles, with simpler checks at each cycle. This is enabled by using tag, and decoupling the store queue into two shift-registers (fig 2a). Some checks need not be performed at all, because we can rely on the order property of shift registers (e.g. in store-to-load forwarding, we can forward the first hit). In the worst case, we would still check every entry but our point is that these checks are not done in a single-cycle CAM. We will clarify this in the paper.
2: Testing our LSQ in Dynamatic would not be fair since the frequency gain of our LSQ would be undone by their scheduling implementation. Also, some of our main contributions are tightly coupled with our compiler passes: tagging of accesses to recover order and speculative LSQ allocations. 
We compare cycle numbers directly with Dynamatic, only frequency and area are compared as overheads vs. the respective vendor baseline. We achieve 3x lower frequency degradation and 21x lower area usage for a LSQ with 32 store entries (table II). Such large differences cannot be attributed to synthesis differences between Vivado and Quartus, but only to fundamental differences in the LSQ architectures.

